New Associations of Gamma-Ray Sources from the Fermi Second Source Catalog

We present the results of an all-sky radio survey between 5 and 9 GHz of the fields surrounding all unassociated gamma-ray objects listed in the Fermi Large Area Telescope Second Source Catalog (2FGL). The goal of these observations is to find all new gamma-ray AGN associations with radio sources >10 mJy at 8 GHz. We observed with the Very Large Array and the Australia Telescope Compact Array the areas around unassociated sources, providing localizations of weak radio point sources found in 2FGL fields at arcmin scales. Then we followed-up a subset of those with the Very Long Baseline and the Long Baseline Arrays to confirm detections of radio emission on parsec-scales. We quantified association probabilities based on known statistics of source counts and assuming a uniform distribution of background sources. In total we found 865 radio sources at arcsec scales as candidates for association and detected 95 of 170 selected for follow-up observations at milliarcsecond resolution. Based on this we obtained firm associations for 76 previously unknown gamma-ray AGN. Comparison of these new AGN associations with the predictions from using the WISE color-color diagram shows that half of the associations are missed. We found that 129 out of 588 observed gamma-ray sources at arcmin scales not a single radio continuum source was detected above our sensitivity limit within the 3-sigma gamma-ray localization. These "empty" fields were found to be particularly concentrated at low Galactic latitudes. The nature of these Galactic gamma-ray emitters is not yet determined.

==> assoctable_short.tex <==
\begin{longtable}{llll}

\caption{First 8 entries of 167 possible associations of 2FGL unassociated sources from literature.
         Table~\ref{tab:assoc} is published in its entirety in the electronic edition. A portion is 
         shown here for guidance regarding its form and content. The source types are: SNR = Supernova 
         Remnant; PSR = Pulsar; XSS = X-ray Binary Star System; BSS = Binary Star System.
\label{tab:assoc}}\\

\toprule
2FGL & Association & Type & Reference \\
\midrule
\endfirsthead

\multicolumn{4}{l}{\scriptsize \tablename\ \thetable{} -- \textit{continued from previous page}} \\[1ex]
\toprule
2FGL & Association & Type & Reference \\
\midrule
\endhead

\multicolumn{4}{r}{\textit{Continued on next page ...}} \\
\endfoot
\endlastfoot
J0002.7+6220 & G116.9+0.2 & SNR? & \citep{2009BASI...37...45G}\\
J0106.5+4854 & PSR J0106+4855 & PSR & \citep{2012ApJ...744..105P}\\
J0128.0+6330 & G126.2+1.6 & SNR? & \citep{2009BASI...37...45G}\\
J0128.0+6330 & G127.1+0.5 & SNR? & \citep{2009BASI...37...45G}\\
J0214.5+6251c & G132.7+1.3 & SNR? & \citep{2009BASI...37...45G}\\
J0218.7+6208c & G132.7+1.3 & SNR? & \citep{2009BASI...37...45G}\\
J0221.4+6257c & G132.7+1.3 & SNR? & \citep{2009BASI...37...45G}\\
J0224.0+6204 & G132.7+1.3 & SNR? & \citep{2009BASI...37...45G}\\
\bottomrule
\end{longtable}


==> table_cat4_short.tex <==
\begin{tabular}{@{}c@{\,\,}c@{\,\,\,}c@{\,\,\,}c@{\,\,\,}c@{\,\,\,}c@{\,}c@{\,\,\,}c@{\,}c@{\,}c@{\,\,\,}c@{\,}c@{\,\,\,}c@{\,}c@{\,}c@{\,\,\,}c@{\,\,\,}c}
\hline
IAU name & 2FGL name & F & $\alpha$ & $\delta$ & $\Delta\alpha$ & $\Delta\delta$ & $F_5$ & $F_7 $ & $F_9$ & $D$ & $N\sigma$ & $F_1$ & $C_1$ & $I_1$ & $I_w$ & Camp. \\
         &      &      & h min s & $\circ$ ' '' & '' & '' & mJy & mJy & mJy & ' & & & & & &\\ 
(1) & (2) & (3) & (4) & (5) & (6) & (7) & (8) & (9) & (10) & (11) & (12) & (13) & (14) & (15) & (16) & (17) \\ 
\hline
J0008+6837 & J0007.7+6825c &  & 00 08 33.31 & +68 37 21.27 & 0.050 & 0.050 & 12.9 & 3.4 & 264.4 & J000833+683721 & N & J000833.39+683722.1 & V1\\
J0031-5511 & J0032.7-5521 &  & 00 31 57.45 & -55 11 46.98 & 2.459 & 3.733 & 11.6 & 8.6 & 18.1 & J003156-551149 & S & J003156.87-551145.1 & A2\\
J0031-5521 & J0032.7-5521 &  & 00 31 02.94 & -55 21 08.69 & 0.360 & 0.493 & 14.2 & 10.2 & 381.2 & J003102-552107 & S & J003102.47-552104.3 & A2\\
J0032-5522 & J0032.7-5521 &  & 00 32 11.00 & -55 22 27.07 & 0.472 & 0.774 & 4.7 & 3.3 & 34.3 & J003210-552228 & S & J003210.93-552227.9 & A2\\
J0032-5525 & J0032.7-5521 &  & 00 32 39.66 & -55 25 48.47 & 1.750 & 2.466 & 4.5 & 3.2 & 13.5 & J003239-552547 & S & J003240.00-552550.1 & A2\\
J0032-5528 & J0032.7-5521 &  & 00 32 54.85 & -55 28 32.77 & 1.238 & 2.153 & 7.4 & 5.3 & -9.9 &  &  & J003255.06-552830.9 & A2\\
J0037+6254 & J0038.8+6259 &  & 00 37 11.29 & +62 54 37.89 & 0.050 & 0.050 & 12.7 & 6.3 & 424.9 & J003711+625439 & N & J003711.36+625438.4 & V1\\
J0047-6347 & J0048.8-6347 &  & 00 47 11.97 & -63 47 50.37 & 0.320 & 0.522 & 11.1 & 3.8 & 290.4 & J004711-634749 & S & J004711.96-634751.7 & A2\\
\hline
\end{tabular}

